Real-time dense 3D Reconstruction from monocular video data captured by low-cost UAVs

Real-time 3D reconstruction enables fast dense mapping of the environment which benefits numerous applications, such as navigation or live evaluation of an emergency. In contrast to most real-time capable approaches, our approach does not need an explicit depth sensor. Instead, we only rely on a video stream from a camera and its intrinsic calibration. By exploiting the self-motion of the unmanned aerial vehicle (UAV) flying with oblique view around buildings, we estimate both camera trajectory and depth for selected images with enough novel content. To create a 3D model of the scene, we rely on a three-stage processing chain. First, we estimate the rough camera trajectory using a simultaneous localization and mapping (SLAM) algorithm. Once a suitable constellation is found, we estimate depth for local bundles of images using a Multi-View Stereo (MVS) approach and then fuse this depth into a global surfel-based model. For our evaluation, we use 55 video sequences with diverse settings, consisting of both synthetic and real scenes. We evaluate not only the generated reconstruction but also the intermediate products and achieve competitive results both qualitatively and quantitatively. At the same time, our method can keep up with a 30 fps video for a resolution of 768x448 pixels.

==> chapters/05_discussion.tex <==
\section{DISCUSSION OF THE EXPERIMENT RESULTS}
\label{sec:discussion}

% KAO: Sloppy spacing ensures non-overfull lines. Can be removed if this is not an issue.
\sloppy 

In the following section, we address relevant properties of our processing chain and put the results presented in  \Cref{sec:eval} in context with each other. %
In particular, we address the circumstances under which 3D model creation might fail and also compare the error measures of the three parts of our approach. %

\subsection{Failed registration and broken model}\label{sec:broken}
As described in \Cref{sec:pose_eval}, our approach does not yield a useful result on 7.85\% of the synthetic sequences. %
This is mainly due to the fact that the registration of depth maps fails because of difficult scenery. %
If this happens once with subsequent correct registration, this will not be critical since these outliers can be eliminated over time by sufficient correct values. %
Repeated incorrect registrations result in a very noisy model, which makes subsequent correct registrations even more difficult. %
Since our fusion approach uses a global model that integrates all depth maps, there is currently no way to recover from this state. %

In edge cases, such as rapid camera movements, if depth maps cannot be estimated over a certain period of time, it is difficult to register the next depth map into the global model due to insufficient overlap. % 
We therefore depend on the sampling of images suitable for depth estimation at regular intervals. %
Our experiments have also shown that scenes with particularly flat terrain and few structures present great difficulties for the registration. %

Depending on the application scenario and the type of depth estimation, softening the sampling criteria may also be an option. %
For this purpose, the capabilities of the depth estimation must be known beyond the optimal parameters in order to determine up to which limit acceptable values are still generated. %
In this case, one would prioritize further model generation and accept inferior depth maps with accompanying noise in the 3D model. %
However, if quality is more important, it should be detected in real-time that the model has an error, \eg to adjust further flight parameters. %

\subsection{Error propagation}
In order to investigate the dynamics of our processing chain and to identify a possible error propagation, we investigate if there are direct dependencies between the errors. %
Depending on the sequence, the \gls*{RMSE} of our point clouds is a poor criterion for a good 3D model. %
Especially in scenes with a lot of flat terrain, models where the registration of the depth maps fails also deliver good results as long as the ground plane is well aligned. %
Consequently, for the detection of completely broken models, the analysis of the camera trajectories is much more meaningful. %

Conversely, a high \gls*{RMSE} of the camera trajectory does not correspond to a high \gls*{RMSE} of the point cloud. %
However, in contrast, the \gls*{RMSE} of the point clouds increases when the quality of the depth maps decreases. %
This corresponds with the subjective impression of more noisy point clouds in sequences with a lower accuracy in depth estimation. %
The fact that we do not observe a similar drop in performance in camera tracking suggests that it is relatively robust against outliers. %

\iffalse

\begin{minipage}{\linewidth}
    \begin{center}
        \includegraphics[width=70mm]{figures/icp_rmse_depth_a5_plot.pdf}
        \small 
        \captionof{figure}{Comparison of evaluation of 3D model generation, depth and trajectory estimation. %
        The graph shows that a decrease in the accuracy of our depth maps is accompanied by an increase in the \gls*{RMSE} of the point cloud.}
        \label{fig:errors}
    \end{center}
\end{minipage}

\fi




==> chapters/07_acknowledgments.tex <==
\section*{ACKNOWLEDGEMENTS}
\label{sec:acknowledgments}
